Propagating gravitons vs. dark matter in asymptotically safe quantum gravity

Within the Asymptotic Safety scenario, we discuss whether Quantum Einstein Gravity (QEG) can give rise to a semi-classical regime of propagating physical gravitons (gravitational waves) governed by an effective theory which complies with the standard rules of local quantum field theory. According to earlier investigations based on single-metric truncations there is a tension between this requirement and the condition of Asymptotic Safety since the former (latter) requires a positive (negative) anomalous dimension of Newton's constant. We show that the problem disappears using the bi-metric renormalization group flows that became available recently: They admit an asymptotically safe UV limit and, at the same time, a genuine semi-classical regime with a positive anomalous dimension. This brings the gravitons of QEG on a par with arbitrary (standard model, etc.) particles which exist as asymptotic states. We also argue that metric perturbations on almost Planckian scales might not be propagating, and we propose an interpretation as a form of `dark matter'.

==> globalDefinitions.tex <==
\makeatletter
\renewcommand*\env@matrix[1][*\c@MaxMatrixCols c]{%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{#1}}
\makeatother

\makeatletter
\def\hlinewd#1{%
\noalign{\ifnum0=`}\fi\hrule \@height #1 %
\futurelet\reserved@a\@xhline}
\makeatother

% \usepackage[printonlyused]{acronym}

\renewcommand{\vec}[1]{\boldsymbol{#1}}
\renewcommand{\epsilon}{\varepsilon}

\newcommand{\sP}[2]{\left(#1,#2\right)}
\newcommand{\fsp}{\mathds{F}_{\Phi}}
\newcommand{\makeNote}{\marginpar[\hfill \color{red} $\longrightarrow$]{\color{red}$\longleftarrow$\hfill}}
\newcommand{\sM}{\mathcal{G}[\bar{\Phi}]}
\newcommand{\sMg}{G[\bar{\Phi}]}

% Sum+ Integral symbol
\DeclareMathOperator*{\SumInt}{%
\mathchoice%
  {\ooalign{$\displaystyle\sum$\cr\hidewidth$\displaystyle\int$\hidewidth\cr}}
  {\ooalign{\raisebox{.14\height}{\scalebox{.7}{$\textstyle\sum$}}\cr\hidewidth$\textstyle\int$\hidewidth\cr}}
  {\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
  {\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
}


\newcommand{\vfb}{V}

%Reference-Punkte
\newcommand{\refpoint}[3]{\begingroup \begin{parcolumns}[colwidths={1=0.3cm},nofirstindent=true]{2}\colchunk{}%
\colchunk{ \raggedright {\sffamily \bf \fontsize{12pt}{12pt}\selectfont #2 }\\ {\rmfamily \fontsize{12pt}{12pt}\selectfont \hspace{0.05cm} #1 \, , \, \cite{#3}.}\linebreak } \end{parcolumns}\endgroup}
\newcommand{\RegA}{R}


\newcommand{\cix}{I}

%Cutoff-Operator
\newcommand{\CutO}{{\cal R}}
\newcommand{\CutM}{R}


% \newcommand{\iou}[2]{\genfrac{(}{)}{0pt}{3}{\mkern-3mu#1\mkern-2.5mu}{\mkern-3mu#2\mkern-2.5mu}}
 \newcommand{\iou}[2]{{\scriptscriptstyle \underline{\bm{(}\mkern-1.5mu#1;#2\bm{)}\mspace{-3.0mu}}\mspace{3.0mu}}}
\newcommand{\ivC}[1]{\mspace{-1.5mu}\underline{\boldsymbol{#1}\mspace{-3.0mu}}\mspace{3.0mu}}
\newcommand{\ivc}[2]{\ivC{#1}}
\newcommand{\basisSet}{{\cal B}}
\newcommand{\be}[2]{e_{\iou{#1}{#2}}}
\newcommand{\bE}[2]{E_{\,\ivc{#1}{#2}}}
\newcommand{\bEi}[2]{E_{\iou{#1}{#2}}}
\newcommand{\bEp}[3]{E^{\mSE(#3)}_{\ivc{#1}{#2}}}
\newcommand{\bEpi}[3]{E^{\mSE(#3)}_{\iou{#1}{#2}}}
% \newcommand{\bE}{E}
 \newcommand{\ip}[3]{\left(#1 | #2 \right)_{#3}}

%roman numbers
\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

%Textbausteine im Mathemodus

\newcommand{\arbit}{\text{arbitrary}}
\newcommand{\selfcon}{\text{selfcon}}
\newcommand{\sCon}{\text{sc}}
\newcommand{\crit}{\text{crit}}


%###############################################################################
%    MATHEMATIK
%###############################################################################
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Zahlenbereiche & Räume
\newcommand{\noR}{\mathds{R}}
\newcommand{\noN}{\mathds{N}}
\newcommand{\noC}{\mathds{C}}
\newcommand{\noZ}{\mathds{Z}}
\newcommand{\Hoe}[2]{C^{#1 , #2}} %Hoelder-Raum
\newcommand{\SteC}[1]{C^{#1}}
\newcommand{\Tens}[3]{\mathcal{T}^{#1}_{#2}{(#3)}}
\newcommand{\On}[1]{O(#1)}
\newcommand{\SOn}[1]{SO(#1)}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Differential-Geometrie
\newcommand{\Lie}{\mathscr{L}}  %Lie-Ableitung
\newcommand{\MaF}{\mathcal{M}} %Integrations-Riemann-Mannigfaltigkeit
\newcommand{\bsl}{\backslash}
%g-bar
\newcommand{\MaFs}{\mathcal{M}}  %Allgemeine Riemann-Mannigfaltigkeit
\newcommand{\MIF}{\mathcal{N}_{\hyp}}
\newcommand{\SymSet}{\text{Sym}[\Tens{0}{2}{\MaFs}]}
\newcommand{\SymSets}{\text{Sym}}
\newcommand{\TM}{\mathcal{T}}  %tangential space
\newcommand{\VF}{\mathscr{T}^1_0} %space of vectorfields
\newcommand{\coDif}{\updelta}
\newcommand{\Dif}{\text{d}}
\newcommand{\Indx}{\text{\tiny index}}
\newcommand{\Hstar}{\star}
\newcommand{\kForm}[2]{\stackrel{\text{\tiny #2}}{#1}\,}
\newcommand{\harmF}{\mathcal{H}}
\newcommand{\sym}[1]{\text{sym}\left[#1\right]}
%\newcommand{\Lie}[1]{\mathscr{L}_{#1}}
\newcommand{\LieBra}[2]{\left[#1;#2\right]_{\mathscr{L}}}
\newcommand{\tp}{\mathcal{T}}
\newcommand{\mx}{\mathcal{X}}
\newcommand{\vecSp}{X}
\newcommand{\TgSp}[2]{T_{#2} #1}
\newcommand{\TSp}[1]{T #1}
\newcommand{\atlas}{\mathcal{A}}
\newcommand{\Christ}[3]{\left\{\genfrac{}{}{0pt}{1}{#1}{#2\, #3}\right\} }
%Legendre Fennel- Transform 
\newcommand{\LFT}[1]{\text{LFT}\left\{#1\right\}}
\newcommand{\txLFT}{{\bf LFT }}
\newcommand{\LT}[1]{\text{LT}\left\{#1\right\}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Geometrische Objekte
\newcommand{\Ric}{R}     % Ricci tensor
\newcommand{\Rm}{R}     % Riemann tensor
\newcommand{\SR}{R}     % Scalar curvature
\newcommand{\EinT}{G}    %Einstein tensor
\newcommand{\bEinT}{\bar{G}}   %Einstein tensor bar
\newcommand{\Ricb}{\bar{\Ric}}     % Ricci tensor
\newcommand{\Rmb}{\bar{\Rm}}     % Riemann tensor
\newcommand{\SRb}{\bar{\SR}}     % Scalar curvature
\newcommand{\Z}{D}      % connection
\newcommand{\ZH}{\text{D}}      % connection
\newcommand{\CoC}[3]{\Gamma_{#2 #3}^{#1}}  %Connection Coefficient}
\newcommand{\CoCbar}[3]{\overline{\Gamma}_{#2 #3} ^{#1}} %Connection
%Coefficient}
\newcommand{\CoCA}[6]{\widetilde{\Gamma}_{\text{g}}\left[#5\right]_{#2 #3} ^{#1}} %general
%Connection Coefficient}
\newcommand{\Cris}[4]{\frac{1}{2} g^{#1 #4} \left(\partial_{#2}g_{#4
#3}+\partial_{#3}g_{#2 #4}-\partial_{#4}g_{#2 #3}\right)}
\newcommand{\CrisA}[7]{\frac{1}{2} #5^{#1 #4} \left(#7_{#2}#6_{#4
#3}+#7_{#3}#6_{#2 #4}-#7_{#4}#6_{#2 #3}\right)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Felder
\newcommand{\bg}{\bar{g}}   %Metric
\newcommand{\bZ}{\bar{\Z}}   %Connection
\newcommand{\bgm}{\bg}
\newcommand{\flH}{\hat{h}}		%fluctuation metric 
\newcommand{\hb}{\bar{h}}
\newcommand{\hx}{h}
\newcommand{\hhat}{\tilde{h}}   %traceless part of h
\newcommand{\htr}{\phi}
%transversal-traceless part
%------------------------------------------------------------------------------
%Oberflaeche
\newcommand{\iM}{H}  %induzierte Metrik auf der Oberfläche
\newcommand{\EC}{K}  % extrinsic curvature
%------------------------------------------------------------------------------
%GeometryOnSurface kapitel
\newcommand{\hyp}{\mathcal{H}}		%hyperplane
\newcommand{\derMat}{B}		%deformation matrix
\newcommand{\matA}{A}		%orthogonal matrix
\newcommand{\tM}{\tilde{t}}		%transverse metric
%------------------------------------------------------------------------------
%Critical Hypersurface
\newcommand{\stabM}{B}
\newcommand{\cUV}{\mathscr{S}_{\text{UV}}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Funktions Definitionen
\newcommand{\id}{\delta} % Identity
\newcommand{\idm}{\Eins} % Identity
\newcommand{\var}{\delta} %variation
\newcommand{\com}[2]{\left[#1,#2\right]} % commutator
\newcommand{\varFunc}{\delta}     %functional derivative
%symbol
\newcommand{\fD}[2]{\frac{\varFunc #1}{\varFunc #2}} % functional derivative
\newcommand{\fDn}[3]{\frac{\varFunc^{#3} #1}{\varFunc #2}} %functional nth
%derivative
\newcommand{\sgn}{\text{sgn}}  %signum
\newcommand{\adj}{\,\text{adj}}  %adjoint
\newcommand{\tr}{\text{tr}}   %trace
\newcommand{\Tr}{\text{Tr}}   %functional Trace
\newcommand{\Order}[1]{\mathcal{O}\left(#1\right)}  %Ordnung
\newcommand{\OrderX}[2]{\mathcal{O}^{#2}(#1)}
\newcommand{\epsTen}{\varepsilon}						%{{\Large\text{$\upvarepsilon$}}}
\newcommand{\GF}[1]{\Gamma\left(#1\right)}   %Gamma-function
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Differentialoperatoren
\newcommand{\Quabla}{\hbox{\footnotesize{$\Box$}}} % D'Alembert
\newcommand{\Laplace}{\Delta}
\newcommand{\Ellipt}{\Delta_E}
\newcommand{\LaB}{\Box}    %Laplace-Beltrami operator
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Integration
\newcommand{\IntSp}[2]{\int \md^{#1} #2 \,} %spacetime-integral dimension #1
\newcommand{\IntSpI}[2]{\int^{#1}_{#2} }  %spacetime-integral
%dimension #1
\newcommand{\IntSpM}[3]{\int_{#3} d^{#1} #2 \,} %spacetime-integral dimension #1
%restricted on #3
\newcommand{\IntSpMs}[3]{\int^{#2}_{#3}} %spacetime-integral dimension #1
\newcommand{\PI}{\mathcal{PI}}   %partielle Integration
\newcommand{\md}{\text{\rm d}} %integral measure variables
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Distribution
\newcommand{\DisD}[1]{\delta\left(#1\right)}  %Delta Distribution
\newcommand{\DisDr}[1]{\delta\left[#1\right]}  %Delta Distribution of Functionals
\newcommand{\kDelta}{\delta}	%Kronecker Delta
\newcommand{\Heaviside}[1]{\Theta \left(#1\right)} %Heaviside
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%HILFSDEFINITIONEN
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commands for the second variation of the Riemann tensor
\newcommand{\CTaF}[7]{\Rm_{#1 #2 #5}\,^{#6}\var g_{#6
#7}\left(\id_{#3}^{#5}\id_{#4}^{#7}+\id_{#3}^{#7}\id_{#4}^{#5}\right)}
\newcommand{\Ida}[4]{\left(\id_{#1}^{#3}\id_{#2}^{#4}+\id_{#1}^{#4}\id_{#2}^{#3}
\right)}
\newcommand{\CTbF}[4]{\Z_{#1}\Z_{#3}h_{#2 #4} - \Z_{#2}\Z_{#3}h_{#1 #4} -
\Z_{#1}\Z_{#4}h_{#2 #3} + \Z_{#2}\Z_{#4}h_{#1 #3}}
\newcommand{\CTbS}[8]{\left[\id^{#5}_{#1}
\id^{#6}_{#3}\id^{#7}_{#4}\id^{#8}_{#2} - \id^{#5}_{#2}
\id^{#6}_{#3}\id^{#7}_{#4}\id^{#8}_{#1}-\id^{#5}_{#1}
\id^{#6}_{#4}\id^{#7}_{#3}\id^{#8}_{#2} + \id^{#5}_{#2}
\id^{#6}_{#4}\id^{#7}_{#3}\id^{#8}_{#1}\right]\Z_{#5}\Z_{#6}\left(\var g_{#7
#8}\right)}
\newcommand{\CTbSF}[8]{\left(\id^{#5}_{#1}
\id^{#6}_{#3}\id^{#7}_{#4}\id^{#8}_{#2} - \id^{#5}_{#2}
\id^{#6}_{#3}\id^{#7}_{#4}\id^{#8}_{#1}-\id^{#5}_{#1}
\id^{#6}_{#4}\id^{#7}_{#3}\id^{#8}_{#2} + \id^{#5}_{#2}
\id^{#6}_{#4}\id^{#7}_{#3}\id^{#8}_{#1}\right)}
\newcommand{\CTbST}[8]{\left[\id^{#5}_{#1}
\id^{#6}_{#2}\id^{#7}_{#3}\id^{#8}_{#4} - \id^{#5}_{#4}
\id^{#6}_{#2}\id^{#7}_{#3}\id^{#8}_{#1}-\id^{#5}_{#1}
\id^{#6}_{#3}\id^{#7}_{#4}\id^{#8}_{#2} + \id^{#5}_{#4}
\id^{#6}_{#3}\id^{#7}_{#2}\id^{#8}_{#1}\right]\Z_{#5}\Z_{#6}\left(\var g_{#7
#8}\right)}
\newcommand{\CTbSTF}[8]{\left[\id^{#5}_{#1}
\id^{#6}_{#2}\id^{#7}_{#3}\id^{#8}_{#4} - \id^{#5}_{#4}
\id^{#6}_{#2}\id^{#7}_{#3}\id^{#8}_{#1}-\id^{#5}_{#1}
\id^{#6}_{#3}\id^{#7}_{#4}\id^{#8}_{#2} + \id^{#5}_{#4}
\id^{#6}_{#3}\id^{#7}_{#2}\id^{#8}_{#1}\right]}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematik-Umgebungen und Formate
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstaende
\newcommand{\SepFE}{\vspace{-0.5cm}} %Separation 1. Zeile Rest
\newcommand{\SepFe}{\vspace{-0.4cm}} %Separation 1. Zeile Rest
\newcommand{\SepSR}{\vspace{-1cm}} %Separation SideNote Rest
\newcommand{\SNW}{1.5cm} %Weite von linkem Rand Sidenote
\newcommand{\SSNW}{2.5cm} %Weite von linkem Rand Sub-Side-Note
\newcommand{\NMW}{1cm} % Weite von linkem Rand normale Formel
\newcommand{\FEW}{0.3cm} %Weite von linkem Rand first Equation
\newcommand{\SDNW}{1.5cm} %Weite von linkem Rand Herleitung
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Allgemeine Symbole
\newcommand{\Ii}{\mathrm{i}}      
%imaginary number
\newcommand{\LHS}{\text{LHS}}     
%LHS
\newcommand{\RHS}{\text{RHS}}     
%RHS
\newcommand{\QED}{\begin{flushright} \color{Text} $\Box$ \end{flushright}}
%q.e.d.
\newcommand{\Res}{\text{Res}}     
%Residium
\newcommand{\xfrac}[2]{%     
%Bruch mit schrägstrich
\mbox{\raisebox{0.4ex}{\ensuremath{\displaystyle #1}\hspace{0.2ex}}%
{\raisebox{-0.1ex}{\Large /}}%
\raisebox{-0.2ex}{\ensuremath{\displaystyle #2}}%
}%
}
\newcommand{\const}{\text{const}}    
%const
%\newcommand{\ker}{\text{ker}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Umformungs-operationen
\newcommand{\cancl}[2]{#2}%{\color{#1} \cancel{#2}}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Umgebungen
%  neuer  Befehl:  \includegraphicstotab[..]{..}
%  Verwendung  analog  wie  \includegraphics
% \newlength{\myx}  %  Variable  zum  Speichern  der  Bildbreite
% \newlength{\myy}  %  Variable  zum  Speichern  der  Bildh�he
% \newcommand\includegraphicstotab[2][\relax]{%
% %  Abspeichern  der  Bildabmessungen
% \settowidth{\myx}{\includegraphics[{#1}]{#2}}%
% \settoheight{\myy}{\includegraphics[{#1}]{#2}}%
% %  das  eigentliche  Einf�gen
% \parbox[c][1.1\myy][c]{\myx}{%
% \includegraphics[{#1}]{#2}}%
% }%  Ende  neuer  Befehl

%-------------------------------------------------------------------------------
% % Central equation
%Farben
\definecolor{shadecolor}{rgb}{0.98,.98,1}
\definecolor{framecolor}{rgb}{0.5,0.5,1}
\definecolor{shadecolorII}{rgb}{0.98,0.98,0.98}
\definecolor{framecolorII}{rgb}{0.6,0.6,0.6}


\newenvironment{bshaded}{%
 \def\FrameCommand{\fcolorbox{framecolor}{shadecolor}}%
 \MakeFramed {\FrameRestore}}%
 {\endMakeFramed}

\newenvironment{bshadedII}{%
 \def\FrameCommand{\fcolorbox{framecolorII}{shadecolorII}}%
 \MakeFramed {\FrameRestore}}%
 {\endMakeFramed}

\newenvironment{bCentralEqn}{%
 \begin{bshaded}\csname align\endcsname}{\csname endalign \endcsname{bshaded}}
 
%-------------------------------------------------------------------------------
% Standard-Formel-Umgebung Herleitung ohne betonung der ersten Zeile
\newenvironment{FormelnE}{\color{Formel} \allowdisplaybreaks
\setlength{\mathindent}{\NMW}\csname align*\endcsname}
{\csname endalign*\endcsname \setlength{\mathindent}{\FEW}\color{Text} }
%-------------------------------------------------------------------------------

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Umgebungen für spezielle Problematiken
%-------------------------------------------------------------------------------
%Eigenwertgleichungen
\newcommand{\EigProb}[2]{\begin{align} & { \bf \color{Formel}\text{Equation} }&
& {\bf \color{Formel}\text{Constraints} }\nonumber \\ & #1 & & #2 \end{align}}
%-------------------------------------------------------------------------------
%Lösungsgleichungen
\newcommand{\SolProb}[3]{\begin{align} & { \bf \color{Formel}\text{Solution} }&
& {\bf \color{Formel}\text{Constraints} }\nonumber \\ & #1 & & #2 \nonumber \\ &
& & #3 \end{align}}
%-------------------------------------------------------------------------------
%Allgemeines Problem1
\newcommand{\GenProb}[4]{\begin{align} & { \bf \color{Formel}\text{#1} }& & {\bf
\color{Formel}\text{#2} }\nonumber \\ & #3 & & #4 \end{align}}
%-------------------------------------------------------------------------------
%Allgemeines Problem2
\newcommand{\GenProbA}[8]{\begin{align} & { \bf \color{Formel}\text{#1} }& &
{\bf \color{Formel}\text{#2} }\nonumber \\ & #3 & & #4 \\ & { \bf
\color{SideNote}\text{#5} }& & {\bf \color{SideNote}\text{#6} }\nonumber \\ & #7
& & #8 \end{align}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Umgebungen für Zusammenfassungen
%-------------------------------------------------------------------------------
% Weyl-Transformation -Zusammenfassungspunkt (Weyl-Transformierte ist #2 mit
%überdach)
\newcommand{\SumWeyl}[4]{\noindent $\bullet$ \text{\color{Formel} #1} 
\begin{align}
\begin{array}{ll} \widetilde{#2} &=  #3  \\ 
\frac{\md}{\md\epsilon}\left.  \widetilde{#2} \right|_{\epsilon=0} &=  #4
\end{array}\end{align}}
% % -------------------------------------------------------------------------------
% % Weyl-Transformation -Zusammenfassungspunkt (Weyl-Transformierte ist #2 mit
% % überdach)
% \newcommand{\SumWeyl}[4]{\noindent \colorbox{Formel}{\parbox{0.5
% cm}{\color{Formel} --}} \quad  \text{\color{Formel} #1}
% \begin{align}\color{Text} \widetilde{#2} &= \color{SumWeylCol} #3 \nonumber  \\ 
% &\color{Text} \stackrel{\Order{\epsilon}}{\simeq} \color{SumWeylCol} #4
% \end{align}}
% %-------------------------------------------------------------------------------
% %Weyl-Transformation -Zusammenfassungspunkt (Weyl-Transformierte ist #5)
% \newcommand{\SumWeylb}[5]{\noindent \colorbox{Formel}{\parbox{0.5
% cm}{\color{Formel} --}} \quad  \text{\color{Formel} #1}
% \begin{align}\color{Text} #5 &= \color{SumWeylCol} #3 \nonumber  \\ 
% &\color{Text} \stackrel{\Order{\epsilon}}{\simeq} \color{SumWeylCol} #4
% \end{align}}
%-------------------------------------------------------------------------------
%Weyl-Transformation -Zusammenfassungspunkt (Weyl-Transformierte ist #5)
\newcommand{\SumWeylb}[5]{\noindent $\bullet$ \text{\color{Formel} #1}
\begin{align}
\begin{array}{ll} #5 &=  #3  \\ 
\frac{\md}{\md\epsilon}\left.  #5 \right|_{\epsilon=0} &=  #4
\end{array}\end{align}}
%-------------------------------------------------------------------------------
%Variations -Zusammenfassungspunkt (1. Variation von #2)
\newcommand{\SumGeo}[4]{\noindent \colorbox{Formel}{\parbox{0.5
cm}{\color{Formel} --}} \quad  \text{\color{Formel} #1}
\begin{align*}\color{Text} \var \left( #2 \right) &= \color{SumGeoCol} #3
\tag*{(#4)} \end{align*}}
%-------------------------------------------------------------------------------
%Variations -Zusammenfassungspunkt (2. Variation von #2)
\newcommand{\SumGeoS}[4]{\noindent \colorbox{Formel}{\parbox{0.5
cm}{\color{Formel} --}} \quad  \text{\color{Formel} #1}
\begin{align*}\color{Text} \var^2 \left( #2 \right) &= \color{SumGeoCol} #3
\tag*{(#4)} \end{align*}}
%-------------------------------------------------------------------------------
%Variations -Zusammenfassungspunkt (2. Variation von #2)
\newcommand{\SumGeoSp}[4]{\noindent \colorbox{Formel}{\parbox{0.5
cm}{\color{Formel} --}} \quad  \text{\color{Formel} #1}
\begin{align*}\color{Text} \var^2 &\left( #2 \right)\\ &= \color{SumGeoCol} #3
\tag*{(#4)} \end{align*}}
%-------------------------------------------------------------------------------
%Variations -Zusammenfassungspunkt (2. Variation von #2)
\newcommand{\PointL}[3]{\noindent {\bf \color{Formel} #1 } \\ #2 \begin{align*}
&{\bf \color{SideNote} \text{ Special cases}} \\ & #3 \end{align*}}
%-------------------------------------------------------------------------------
%Variations -Zusammenfassungspunkt (2. Variation von #2)
\newcommand{\SubPointL}[2]{ \quad \text{#1} & \Rightarrow & #2}
%-------------------------------------------------------------------------------
%Weyl-Transformation -Zusammenfassungspunkt (Weyl-Transformierte ist #5)
\newcommand{\SumWeylC}[4]{\noindent \colorbox{Formel}{\parbox{0.5
cm}{\color{Formel} --}} \quad  \text{\color{Formel} #1}
\begin{align}\color{Text} #2 &= \color{SumWeylCol} #3 \nonumber  \\ 
&\color{Text} \simeq \color{SumWeylCol} #4  \end{align}}
%-------------------------------------------------------------------------------
%Weyl-Transformation -Zusammenfassungspunkt (Weyl-Transformierte ist #5)
\newcommand{\SumWeylD}[3]{\noindent \colorbox{Formel}{\parbox{0.5
cm}{\color{Formel} --}} \quad  \text{\color{Formel} #1}
\begin{align}\color{Text} #2 &= \color{SumWeylCol} #3 \end{align}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Physikalische Objekte
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%-------------------------------------------------------------------------------
%Wirkung
 
\newcommand{\SW}{S}  %Action
\newcommand{\ISW}{{\cal I}} 	%Integral part of Action 
\newcommand{\EA}{\Gamma}
\newcommand{\EAA}{\Gamma}  %Effective Average action
\newcommand{\CGF}{W}   %connected generating funcntional
\newcommand{\La}{\mathcal{L}}  %range density
\newcommand{\ParF}{\text{Z}}  %Partition function
 \newcommand{\ParFD}{\mathds{Z}}  %Partition function
 \newcommand{\frEny}{F}				%{\mathds{F}} 
%-------------------------------------------------------------------------------
%Felder
 
\newcommand{\Gh}{C}   %Ghost Faddeev-Popov
\newcommand{\GhA}{\bar{C}}  % Anti-Ghost
\newcommand{\Ghx}{\xi}   %Expectation Ghost Faddeev-Popov
\newcommand{\GhAx}{\bar{\xi}}  %Expectation Anti-Ghost
 
 
%-------------------------------------------------------------------------------
%Kosmologische Konstante
 
\newcommand{\CosmConst}{\lambda}
%
\newcommand{\Kk}{\CosmConst}  %Kosmologische Konstante (dim-less)
\newcommand{\Kkbar}{\Lambda}  % bare cosmological constant

\newcommand{\cf}{\Omega}

\newcommand{\KkbartD}{\Kkbar^{\dyn}}
\newcommand{\KkbarD}{\Kkbar_k^{\dyn}}  % bare cosmological constant
\newcommand{\KkbarB}{\Kkbar_k^{\background}}  % bare cosmological constant
%Surface
\newcommand{\KkEC}{\CosmConst^{\partial}}  %Kosmologische Konstante
% (dim-less) dM
\newcommand{\KkbarEC}{\bar{\CosmConst}^{\partial}}  % bare
%cosmological constant dM

\newcommand{\Kka}{\CosmConst_{1;k}}  %Kosmologische Konstante (dim-less)
\newcommand{\Kkb}{\CosmConst_{2;k}}  %Kosmologische Konstante (dim-less)
\newcommand{\KkECa}{\CosmConst^{\partial}_{1;k}}  %Kosmologische Konstante (dim-less)
\newcommand{\KkECb}{\CosmConst^{\partial}_{2;k}}  %Kosmologische Konstante (dim-less)
 
%-------------------------------------------------------------------------------
%Newtonskonstante

\newcommand{\Nkpd}{\text{g}^{\dyn \dotpart}}  %Newtons Konstante (dim-less)
\newcommand{\Nkd}{\text{g}^{\dyn}}  %Newtons Konstante (dim-less)
\newcommand{\Nk}{G}  %Newtons Konstante 
\newcommand{\Nkbar}{\Nk_N}%{\overline{\text{G}}} %Newtons Konstante bar
%Surface
\newcommand{\NkECd}{\text{g}^{\dyn,\partial}}  %Newtons Konstante
%dim-less
\newcommand{\NkEC}{G^{\partial}}  %Newtons Konstante 
\newcommand{\NkbarEC}{\overline{G}} %Newtons Konstante bar
 
%-------------------------------------------------------------------------------
%Konstanten
 
\newcommand{\kap}{\kappa}
\newcommand{\kapEC}{\kappa}
%
\newcommand{\CcM}{C_{M}}  %C_V constante p.18 M.R.
\newcommand{\CcT}{C_{\hhat}}  %C_T constante p.17 M.R.
\newcommand{\CcS}{C_{\htr}}  %C_S constante p.17 M.R.
%
\newcommand{\CHyp}{\varpi}%C_{\text{Hyp}}}
 
%-------------------------------------------------------------------------------
%Funktionen
 
%Treshold
\newcommand{\Thrf}[5]{\Phi^{#1 ; #3}_{#2}\left(#4,#5\right)}
%Threshold-function
\newcommand{\ThrfA}[3]{\Phi^{#1}_{#2}\left({#3}\right)}
\newcommand{\ThrfAn}[4]{\Phi^{#1\,{\scriptscriptstyle (0,#4,0)}}_{#2}\left({\scriptstyle #3}\right)}
\newcommand{\ThrfBn}[4]{\widetilde{\Phi}^{#1\,{\scriptscriptstyle (0,#4,0)}}_{#2}\left({\scriptstyle #3}\right)}
\newcommand{\qA}[3]{q^{#1}_{#2}\left({#3}\right)}  
\newcommand{\qAn}[4]{q^{#1\,{\scriptscriptstyle (0,#4,0)}}_{#2}\left({\scriptstyle #3}\right)}  
%Threshold-function
\newcommand{\ThrfB}[3]{\widetilde{\Phi}^{#1}_{#2}\left({#3}\right)}
%Threshold-function
\newcommand{\GThrf}[5]{\Upsilon^{#1 ; #3}_{#2}\left(#4,#5\right)}
%generalized Threshold-function
\newcommand{\GThrfA}[4]{\Upsilon^{#1}_{#2 ; #4}\left(#3\right)} 
%generalized Threshold-function
\newcommand{\GThrfB}[4]{\widetilde{\Upsilon}^{#1}_{#2 ; #4}\left(#3\right)} 	
%generalized Threshold-function
%Trace-Abbreviations
\newcommand{\Af}{\mathcal{A}}
\newcommand{\Nf}{\mathcal{N}}
%
\newcommand{\BTfA}[1]{B_{\Phi}\left(#1 \right)}
\newcommand{\BTfB}[1]{B_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\BTfAEC}[1]{B^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\BTfBEC}[1]{B^{\partial}_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\DTfA}[1]{b_{\Phi}\left(#1 \right)}
\newcommand{\DTfB}[1]{b_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\DTfAEC}[1]{b^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\DTfBEC}[1]{b^{\partial}_{\widetilde{\Phi}}\left(#1 \right)}
%Bimetric
\newcommand{\BBTfA}[1]{\overline{B}_{\Phi}\left(#1 \right)}
\newcommand{\BBTfB}[1]{\overline{B}_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\BBTfAEC}[1]{\overline{B}^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\BBTfBEC}[1]{\overline{B}^{\partial}_{\widetilde{\Phi}}
\left(#1\right)}
\newcommand{\BDTfA}[1]{\overline{b}_{\Phi}\left(#1 \right)}
\newcommand{\BDTfB}[1]{\overline{b}_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\BDTfAEC}[1]{\overline{b}^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\BDTfBEC}[1]{\overline{b}^{\partial}_{\widetilde{\Phi}}\left(#1\right)}
%
\newcommand{\CDel}[2]{\text{c}_{#1}^{#2}}
%Mass-Dimension
\newcommand{\Mdim}[1]{\left[#1\right]}  %mass-dimension
 
%-------------------------------------------------------------------------------
%Bimetric


\newcommand{\ph}{{\scriptscriptstyle \#}}
\newcommand{\agf}{\hat{\alpha}}
\newcommand{\ags}{\hat{\alpha}^{\text{new}}}

\newcommand{\sRM}{\text{Riem}}

\newcommand{\DThrfA}[3]{\zeta^{#1\,(#3)}_{#2}}
% \newcommand{\rhoN}{\rho_{\text{grav}}}
\newcommand{\rhoN}{}
\newcommand{\rhoG}{\rho_{\text{gh}}}
\newcommand{\rhoGk}{\rho_{\text{gh}\,k}}
\newcommand{\rhoP}{\rho_{\text{P}}}
\newcommand{\rhoD}{\rho_{\text{D}}}
\newcommand{\rhoA}{\gamma}
 
\newcommand{\background}{\text{B}}
\newcommand{\dyn}{\text{Dyn}}
\newcommand{\lin}{\text{lin}}
\newcommand{\sm}{\text{sm}}
%\newcommand{\bm}{\text{bm}}
%

\newcommand{\zh}{A}

\newcommand{\KkB}{\CosmConst^{\background}}  %Kosmologische Konstante
\newcommand{\KkD}{\CosmConst^{\dyn}} %Kosmologische Konstante
% (dim-less)
\newcommand{\KkECB}{\CosmConst^{\partial}_{\background , k}}
%Kosmologische Konstante  (dim-less) dM
% \newcommand{\KkbarB}{\bar{\CosmConst}_{2;k}}
\newcommand{\KkbarBEC}{\bar{\CosmConst}_{2;k}^{\partial}}
%
\newcommand{\ZfacD}{Z^{\dyn}_{k}}
\newcommand{\ZfacGB}{Z^{\background}_{k}}
%
\newcommand{\ZfacB}{Z^{\background}_{k}}
\newcommand{\ZfacBEC}{Z^{\partial}_{2,k}}
%
\newcommand{\ZfacBt}{Z_{k}}
\newcommand{\ZfacBtEC}{Z^{\partial}_{k}}
%
\newcommand{\NkbarB}{\overline{G}^{\background}} %Newtons Konstante bar
 
\newcommand{\NkdB}{\text{g}^{\background}}  %Newtons Konstante
% (dim-less)
%
\newcommand{\NkbarECB}{\overline{G}^{\background}}
\newcommand{\NkECdB}{\text{g}^{\background,\partial}}  %Newtons
% Konstante dim-less
%
\newcommand{\biM}{\bar{\iM}}
\newcommand{\bEC}{\bar{\EC}}
%
\newcommand{\aDzB}{\eta_2}  %anomalous dimension
\newcommand{\aDzECB}{\eta_2^{\partial}}
 
%-------------------------------------------------------------------------------
%Regulator
 
\newcommand{\RegGr}{R^{\text{grav}}} %Regulator grav
\newcommand{\RegGn}{R} %Regulator grav
\newcommand{\RegGh}{R^{\text{gh}}} %Regulator ghost
\newcommand{\RegX}[1]{R^{(0)}\left(#1\right)} %regulator R0
\newcommand{\RegXd}[1]{R^{(0)\prime}\left(#1\right)} %regulator R0 deriv
\newcommand{\RegY}[2]{R_{\text{#2}}^{(0)}\left(#1\right)} %regulator R0
\newcommand{\RegXdot}[1]{\dot{R}^{(0)}\left(#1\right)}
\newcommand{\RegO}{\RegX{\tfrac{-\bZ^2}{k^2}}} %regulator R0
\newcommand{\RegOd}{\RegXd{\tfrac{-\bZ^2}{k^2}}} %regulator R0 partal diff
\newcommand{\RegOpt}{R_{\text{opt}}} %regulator R0
 
%-------------------------------------------------------------------------------
%

\newcommand{\dEps}{\boldsymbol{\delta}^{\text{split}}_{\epsilon}}
% \newcommand{\dEps}{\dEp^{\text{{\bf split}}}}
\newcommand{\dBgt}{\boldsymbol{\delta}^{\text{{B}}}_{v}}

\newcommand{\kA}{A^{\background}}
\newcommand{\kAx}{A^{\cix}}

\newcommand{\kB}{B_1^{\background}}

\newcommand{\kAD}{B_1^{\dyn}}
\newcommand{\kBD}{B_2^{\dyn}}

\newcommand{\dBb}{B_2^{\dyn}}
\newcommand{\dBa}{B_1^{\dyn}}

\newcommand{\bmA}{\mathcal{B}_{11}}
\newcommand{\bmB}{\mathcal{B}_{12}}
\newcommand{\bmC}{\mathcal{B}_{21}}
\newcommand{\bmD}{\mathcal{B}_{22}}
\newcommand{\bmE}{\mathcal{B}_{31}}
\newcommand{\bmF}{\mathcal{B}_{32}}
\newcommand{\bmG}{\mathcal{B}_{41}}
\newcommand{\bmH}{\mathcal{B}_{42}}
\newcommand{\bmI}{\mathcal{B}_{43}}

\newcommand{\attr}{\bullet}
\newcommand{\AttrL}{\text{{\bf (Attr)$^{\background}$}}}
\newcommand{\SolAttr}{\text{Sol}_{\attr}^{\background}}
\newcommand{\fpnD}{{\bf NG$_+^{\dyn}$}}
\newcommand{\fpnDn}{{\bf NG$_-^{\dyn}$}}

\newcommand{\fpgD}{{\bf G$^{\dyn}$}}
\newcommand{\fpnB}{{\bf NG$_+^{\background}$}}
\newcommand{\fpnBn}{{\bf NG$_-^{\background}$}}
\newcommand{\fpgB}{{\bf G$^{\background}$}}

\newcommand{\fpnO}{{\bf NG$_+^{(0)}$}}
\newcommand{\fpgO}{{\bf G$^{(0)}$}}

\newcommand{\fpnBO}{{\bf NG$_+^{\background\slash(0)}$}}
\newcommand{\fpgBO}{{\bf G$^{\background\slash(0)}$}}



\newcommand{\fpC}{{$\oplus$}}
\newcommand{\fpL}{{\bf FP}}

\newcommand{\Prohtr}{P_{\htr}}  % Projector htrace
\newcommand{\Prohhat}{P_{\hhat}} % Projector hhat
 
\newcommand{\ZfacG}{Z_{k}}
\newcommand{\ZfacECG}{Z^{\partial}_{k}}
\newcommand{\NkdG}{\text{g}}
 
\newcommand{\NkECdG}{\text{g}^{\partial}}
\newcommand{\aDzG}{\eta}
 
\newcommand{\aDz}{\eta^{\dyn}}  %anomalous dimension
\newcommand{\Zfac}{Z_{1,k}}
 
 
\newcommand{\aDzEC}{\eta^{\partial} _{\text{N}}}  %anomalous
% dimension
\newcommand{\ZfacEC}{Z^{\partial}_{1,k}}
 
\newcommand{\dotpart}{\cdot \slash \partial}
\newcommand{\IR}{\text{IR}}
\newcommand{\UV}{\text{UV}}
 
%-------------------------------------------------------------------------------
%MATTER INDUCED Variables
 
\newcommand{\PotA}{V(A)}
\newcommand{\PotAk}{V_k(A)}
\newcommand{\PotAkA}{V^{(0)}_k(A)}
\newcommand{\PotAkB}{V^{(1)}_k(A)}
\newcommand{\PotAd}[1]{V^{#1}_k(A)}
\newcommand{\potAk}{v_k(A)}
% \newcommand{\tg}{\text{g}}
\newcommand{\tg}{g}
\newcommand{\tgD}{g^{\dyn}}
\newcommand{\tgB}{g}
\newcommand{\nkA}{G_k^{(0)}}
\newcommand{\nkD}{G_k^{\dyn}}
\newcommand{\nkbB}{G_k^{\background}}
\newcommand{\nkAB}{G_k^{(0,\partial)}}
\newcommand{\nkB}{G_k^{(1)}}
\newcommand{\nkBB}{G_k^{(1,\partial)}}
\newcommand{\kkA}{\Lambda_k^{(0)}}
\newcommand{\kkAB}{\Lambda_k^{(0,\partial)}}
\newcommand{\kkB}{\Lambda_k^{(1)}}
\newcommand{\xiA}{\xia_k}
\newcommand{\xiaS}{\xi^{(0,\partial)}}
\newcommand{\xiAS}{\xiaS_k}
\newcommand{\xibS}{\xi^{(1,\partial)}}
\newcommand{\xiBS}{\xibS_k}
\newcommand{\xiBg}{\xibg_k}
\newcommand{\xiBR}{\xibR_k}
\newcommand{\xia}{\xi^{(0)}}
\newcommand{\xibg}{\xi^{(1,\text{\Rmnum{1}})}}
\newcommand{\xibR}{\xi^{(1,\text{\Rmnum{2}})}}
%\newcommand{\ekA}{\text{E}_k^{(1,\var\sqrt{g})}}
\newcommand{\varbg}[1]{\var^1 \big(#1 \big)[\bg;\flcb]}
\newcommand{\varA}[1]{\var^1 \big(#1 \big)[A;\var A]}
\newcommand{\varAL}[1]{\var^1 \left(#1 \right)[A;\var A]}
\newcommand{\varAA}[1]{\var^2 \big(#1 \big)[A;\var A]}
\newcommand{\varAAL}[1]{\var^2 \left(#1 \right)[A;\var A]}
\newcommand{\eka}{E_k}   %\ekA = 1 + \eka
\newcommand{\ekA}{\text{B}_k^{(1)}}
\newcommand{\ekB}{\text{E}_k^{(1,\var\Z^2)}}
\newcommand{\TOp}[2]{W_{#1}\left(#2;A\right)}
\newcommand{\ns}{n_{\text{s}}}
\newcommand{\bmk}{\bar{m}_k}
\newcommand{\mk}{m_k}
\newcommand{\mkA}{m^{(0)}_k}
\newcommand{\mka}{m^{(0)}}
\newcommand{\mkB}{m^{(0)\,2}_k}
\newcommand{\mkC}{m^{(1)\,2}_k}
\newcommand{\mkb}{m^{(0)\,2}}
\newcommand{\mkc}{m^{(1)\,2}}
\newcommand{\omgB}{\tilde{\Omega}_k}
\newcommand{\omgA}{u_k}
\newcommand{\bomg}{\bar{u}_k}
\newcommand{\polyn}[1]{\text{Polyn}(#1)}
\newcommand{\Nkbart}{G_N}
\newcommand{\NkbartEC}{G_N}
\newcommand{\Kkbart}{\Lambda}
\newcommand{\KkbartEC}{\Lambda^{\partial}} 
 
 
%-------------------------------------------------------------------------------
%-------------------------------------------------------------------------------
%-------------------------------------------------------------------------------
\newcommand{\AS}{A^{\partial}} 

\newcommand{\EAAbulk}{\EAA^{\text{bulk}}}
\newcommand{\EAAS}{\EAA^{\partial}}
\newcommand{\flcb}{h}
\newcommand{\FPop}{\mathcal{M}}
\newcommand{\ud}[2]{^{#1}_{\phantom{#1}#2}}
\newcommand{\du}[2]{_{#1}^{\phantom{#1}#2}}
\newcommand{\Id}{I}
\newcommand{\calE}{{\cal E}}

